Persistence Steenrod modules

It has long been envisioned that the strength of the barcode invariant of filtered cellular complexes could be increased using cohomology operations. Leveraging recent advances in the computation of Steenrod squares, we introduce a new family of computable invariants on mod 2 persistent cohomology termed $Sq^k$-barcodes. We present a complete algorithmic pipeline for their computation and illustrate their real-world applicability using the space of conformations of the cyclo-octane molecule.

==> aux/circle.tex <==
\begin{tikzpicture}[scale=2.3]
	\coordinate (A) at (210: 1);
	\coordinate (B) at (330: 1);
	\coordinate (C) at (90: 1);

	\draw[] (A) node[left] {0} -- (B) node[right] {1} -- (C) node[above] {2} -- (A);
\end{tikzpicture}

==> aux/klein_sphere.tex <==
\newcommand*{\xMin}{0}%
\newcommand*{\xMax}{4}%
\newcommand*{\yMin}{0}%
\newcommand*{\yMax}{4}%
\newcommand*{\Radius}{12pt}%

\begin{tikzpicture}[scale=.8]
\draw[-{Latex[length=2mm]}] (-.5,\yMin)--(-.5,\yMax);
\draw[-{Latex[length=2mm]}] (-.5,\yMin)--(-.5,\yMax-.5);
\draw[-{Latex[length=2mm]}] (4.5,\yMax)--(4.5,\yMin);
\draw[-{Latex[length=2mm]}] (4.5,\yMax)--(4.5,\yMin+.5);

\draw[-{Latex[length=2mm]}] (\xMin, -.5)--(\xMax, -.5);
\draw[-{Latex[length=2mm]}] (\xMin, 4.5)--(\xMax, 4.5);

\draw (0,0)--(0,4)--(4,4)--(4,0)--(0,0);

\draw[dotted] (1,6*\Radius) arc(90:-90:\Radius);
\draw (1,4*\Radius) arc(270:90:\Radius);

\draw (3,6*\Radius) arc(90:-90:\Radius);
\draw[dotted] (3,4*\Radius) arc(270:90:\Radius);

\draw (1,6*\Radius) .. controls (2,2.4) .. (3,6*\Radius);
\draw (1,4*\Radius) .. controls (2,1.6) .. (3,4*\Radius);

\draw[dotted] (1,9*\Radius) arc(90:-90:\Radius);
\draw (1,7*\Radius) arc(270:90:\Radius);
\draw (1,9*\Radius) .. controls (2,9*\Radius) and (2,7*\Radius) .. (1,7*\Radius);

\draw[dotted] (3,3*\Radius) arc(90:-90:\Radius);
\draw (3,1*\Radius) arc(270:90:\Radius);
\draw (3,3*\Radius) .. controls (4,3*\Radius) and (4,1*\Radius) .. (3,1*\Radius);
\end{tikzpicture}

==> sec/cubical.tex <==
\section{Cubical} \label{s:cubical}

In the body of this article we focused on simplicial complexes since they are better known, but the use of persistence modules can also be extended to cubical complexes.
These are similar to simplicial complexes but relying on cubes as basic shapes instead of a simplices.

An \textit{elementary interval} is a subset of $\R$ of the form $[a, a+1]$  or $[a, a] = \{a\}$ for some $a \in \R$, with the first type referred to as \textit{non-degenerate} and the second as \textit{degenerate}. To a non-degenerate elementary interval we assign two degenerate elementary intervals
\begin{equation*}
d^0 [a, a+1] = [a+1, a+1]
\qquad \text{and} \qquad
d^1 [a, a+1] = [a, a].
\end{equation*}
An \textit{elementary cube} $C$ is a product $I_1 \times I_2 \times \cdots$ of elementary interval in $\R^\infty$ with all but finitely many factors equal to $[0, 0]$. If $I_{k_1}, \dots, I_{k_n}$ are its non-degenerate intervals, we refer to $n$ as the \textit{dimension} of the elementary cube and, assuming
\begin{equation*}
k_1 < \cdots < k_{n},
\end{equation*}
define for $i \geq 1$ the following two elementary cubes:
\begin{align*}
d_i^0 C &= I_1 \times \cdots \times d^0 I_{k_i} \times \cdots , \\
d_i^1 C &= I_1 \times \cdots \times d^1 I_{k_i} \times \cdots .
\end{align*}		
A \textit{cubical complex} is a finite set of elementary cubes and a \textit{cubical complex pair} $(X, Y)$ is a pair of cubical complexes such that $Y \subseteq X$.

\textit{The standard $d$-cube} is the cubical complex with a single standard cube
\begin{equation*}
I_1 \times I_2 \times \cdots
\end{equation*}
with
\begin{equation*}
I_k = \begin{cases}
[0, 1] & \text{if } k \leq d, \\
[0, 0] & \text{if } k > d.
\end{cases}
\end{equation*}

Let $(X, Y)$ be a cubical complex pair. The dg modules of \textit{relative chains} and relative \textit{cochains} of this pair are defined in analogy to that of simplicial complex pairs with
\begin{equation*}
\begin{tikzcd}[column sep=normal, row sep=tiny,row sep = 0ex
,/tikz/column 1/.append style={anchor=base east}
,/tikz/column 2/.append style={anchor=base west}
]
C_n(X, Y; \Bbbk) \arrow[r, "\partial_n"] & C_{n-1}(X, Y; \Bbbk) \\
x\ \arrow[r, |->] & \sum_{i = 1}^{n} (-1)^{i-1}(d^0_i x - d^1_i x).
\end{tikzcd}
\end{equation*}
As before we refer to the spacial case $Y = \emptyset$ as \textit{absolute chains and cochains} respectively, and the \textit{relative (absolute) homology and cohomology} of a simplicial pair $(X, Y)$ is defined as the homology of the corresponding dg module.

Let $X$ be a cubical complex and $x \in X_n$. For a disjoint pair of sets $U_0, U_1 \subseteq \{1, \dots, n\}$ with $U_i = \{u_{1} < \cdots < u_{r_i}\}$ for each $i \in \{0,1\}$, we use the notation
\begin{equation*}
d^{\,i}_{U_i}x = d^{s^i(u_1)}_{u_1} \cdots\ d^{s^i(u_r)}_{u_{r_i}}x
\end{equation*}
where for $u \in U_i$
\begin{equation*}
s^i(u) = \begin{cases}
0 & \text{if } \big| \{1,\dots, u\} \setminus U_0 \cup U_1 \big| \equiv i \text{ mod } 2, \\
1 & \text{otherwise}.
\end{cases}
\end{equation*}

\begin{definition} \label{def: cubical cup-i coproducts}	
	The \textit{cubical cup-$i$ coproduct}
	\begin{equation*}
	\Delta_i : C_\bullet(X; \F) \to C(X; \F)^{\otimes 2}_\bullet
	\end{equation*}
	is the linear map defined by
	\begin{equation} \label{equation: cubical cup-i coproducts}
	\Delta_i (x) = \sum d_{U_0}^{\,0} x \otimes d_{U_1}^{\,1} x
	\end{equation}
	where the sum is taken over all disjoint pairs $U_0, U_1 \subseteq \{0,\dots,n\}$ with $|U_0 \cup U_1| = n-k$.
\end{definition}

\begin{figure}
	\begin{algorithm} [H]
		\KwIn{$X$, $k>0$, $\{c^1, \dots, c^m\} \subseteq X$}
		$T =$ empty set\\
		\ForAll{$c^i = I^i_1 \times \cdots \times I^i_N \ \mathrm{and}\ c^j = I^j_1 \times \cdots \times I^j_N$} {
			$I_1,\dots,I_N =$ empty intervals\\
			$counter = 0$\\
			\For{$s=1,\dots,N$} {
				\If {$I^i_s = I_s^j$} {
					set $I_s = I_s^i$ and add $1$ to $counter$
				}
				\ElseIf{$\partial^\eta I_s^i = \partial^\xi I_s^j $} {
					\If{$I_s^i\ \mathrm{deg\ and}\ I_s^i\ \mathrm{nondeg\ and\ } counter =$ ?\\ 
						$\mathbf{or}\ I_s^i\ \mathrm{nondeg\ and}\ I_s^i\ \mathrm{deg\ and\ } counter =$ ?}{
						set $I_s = I^i_s$
					}
					{$\mathbf{else\ break}$}
				} 
				{$\mathbf{else\ break}$}
			}		
		}
		\KwOut{$T$}
		\caption{cStSq}
	\end{algorithm}
	\caption{Cubical Steenrod squares. MISSING CHECK THAT c IN THE COMPLEX...}
\end{figure}

==> sec/duality.tex <==
%!TEX root = ../pers_st.tex

\subsection{Duality}
\label{sec: duality}

In this subsection we explore the relationship between the Steenrod barcodes of persistent relative and absolute cohomology.

The following example illustrates that, unlike the case of regular barcodes \eqref{e:duality of barcodes}, these do not completely determine each other in general.
Let $\rM$ be the M\"{o}ebius band and consider the filtration $\emptyset \to S^1 \to \rM$ where the circle is included as the boundary of $\rM$.
Given that $H^\bullet(\rM, S^1)$ is isomorphic to the reduced absolute cohomology of the real projective plane $\rM/S^1 \cong \R P^2$, and that $\rM$ is homotopy equivalent to its central circle, one can verify that
the Steenrod barcode of absolute cohomology is empty but that of relative cohomology is not.

An important case where the Steenrod barcodes of persistent relative and absolute cohomology determine each other is when there are only finite bars in their regular barcodes.
More precisely, let $X$ be a p.f.d. filtered complex such that either
\[
Bar_{\mathcal H^\bullet_R(X;\, \F)} =
Bar_{\mathcal H^\bullet_R(X;\, \F)}^{\mathrm{fin}}
\]
or, equivalently,
\[
Bar_{\mathcal H^\bullet_A(X;\, \F)} =
Bar_{\mathcal H^\bullet_A(X;\, \F)}^{\mathrm{fin}}.
\]
Then, for integers $k$ and $n$ there is bijection of multisets
\[
\begin{tikzcd}[column sep = normal, row sep=-5
,/tikz/column 1/.append style={anchor=base east}
,/tikz/column 2/.append style={anchor=base west}]
Sq^k Bar_{\mathcal H^n_R(X;\, \F)} \arrow[r, "\cong"] &
Sq^k Bar_{\mathcal H^{n-1}_A(X;\, \F)} \\
(i, j] \arrow[r, |->] &
(i, j].
\end{tikzcd}
\]
This can be seen using the categorical framework of \cite{bauer2020structure}.
We illustrate the argument in an example that contains all the ideas of the proof.
Consider a two stage filtration $\emptyset \to X_1 \to X_2$ and the diagram
\[
\begin{tikzcd}
\xla{\delta_{n+1}} H^{n+1}(X_1) & \arrow[l, "\, i_{n+1}^\ast"'] H^{n+1}(X_2) & \arrow[l, "\, j_{n+1}^\ast"'] H^{n+1} (X_2, X_1) \xla{\delta_{n}} \\
\xla{\delta_{n}} H^{n}(X_1) \arrow[u, "Sq^1"'] & \arrow[l, "i_n^\ast"'] H^{n}(X_2) \arrow[u, "Sq^1"] & \arrow[l, "j_n^\ast"'] H^{n}(X_2, X_1) \arrow[u, "Sq^1"] \xla{\delta_{n-1}} \\
\xla{\delta_{n-1}} H^{n-1}(X_1) \arrow[u, "Sq^1"'] & \arrow[l, "\ i_{n-1}^\ast"'] H^{n-1}(X_2) \arrow[u, "Sq^1"] & \arrow[l, "\ j_{n-1}^\ast"'] H^{n-1}(X_2, X_1) \arrow[u, "Sq^1"] \xla{\delta_{n-2}}
\end{tikzcd}
\]
where the horizontal maps are part of the long exact sequence of the pair $(X_2, X_1)$.
Consider $\beta \in H^n(X_2,X_1)$ with $Sq^1 \beta \neq 0$.
Since all regular bars are finite we have that $j^\ast_n \, \beta = 0$ so $j^\ast_{n+1} Sq^1 \beta = 0$ and we have an $Sq^1$-bar $(0, 1]_R^{n}$.
By exactness, $\delta_{n-1} \alpha = \beta$ for some $\alpha \in H^{n-1}(X_1)$ where $\delta_{n-1}$ is the $(n-1)^\th$ connecting homomorphism.
Since these commute with Steenrod squares, we have $Sq^1 \alpha \neq 0$.
Furthermore, $Sq^1 \alpha$ is not in the image of $i_n^\ast$ since otherwise $Sq^1 \beta$ would be $0$.
Therefore, there is a $Sq^1$-bar $(0,1]_A^{n-1}$.

Conversely, given $\alpha \in H^{n-1}(X_1)$ with $Sq^1 \alpha \neq 0$ the finiteness assumption implies that $\delta_n \, Sq^1 \alpha \neq 0$ so we have a $Sq^1$-bar $(0,1]_A^{n-1}$.
Denote by $\beta$ the element $\delta_{n-1} \alpha$ and notice that $Sq^1 \beta \neq 0$ with exactness implying $j_n^\ast Sq^1 \beta = 0$, so we have a $Sq^1$-bar $(0,1]_R^{n}$.

A similar diagram chase can be used to show that for arbitrary p.f.d. filtered complexes infinite Steenrod bars correspond under a multiset bijection given by
\[
\begin{tikzcd}[column sep = normal, row sep=-3
,/tikz/column 1/.append style={anchor=base east}
,/tikz/column 2/.append style={anchor=base west}]
Sq^k Bar^{\mathrm{inf}}_{\mathcal H^n_R(X;\, \F)} \arrow[r, "\cong"] &
Sq^k Bar^{\mathrm{inf}}_{\mathcal H^{n}_A(X;\, \F)} \\
(-\infty, k] \arrow[r, |->] &
(k, +\infty].
\end{tikzcd}
\]

We remark that the example $S^1 \to \rM$ shows that finite Steenrod bars associated to infinite regular bars need not correspond.

==> sec/legacy.tex <==
%We remark that the example $S^1 \to \rM$ at the beginning of this subsection shows that finite Steenrod bars associated to infinite regular bars need not correspond between persistent relative and absolute cohomology.

\begin{comment} simplicial map
A \textit{simplicial map} between simplicial complexes is a function between their vertices such that the image of any simplex via the induced map is a simplex.
\end{comment}


\begin{comment}
with induced restriction map $\rho$ make diagram \eqref{e:naturality of Steenrod squares} commute, since, considering an arbitrary representative $\alpha$ of a class $[\alpha] \in H^n(X, Y;\F)$, we have

% restriction symbol
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
\left.\kern-\nulldelimiterspace % automatically resize the bar with \right
#1 % the function
\vphantom{\big|} % pretend it's a little taller at normal size
\right|_{#2} % this is the delimiter
}}
\begin{align*}
\rho \circ Sq^k \big([\alpha]\big) & =
\left[(\alpha \otimes \alpha) \restr{\Delta_{n-k}(-)}{C_{n+k}(X', Y';\F)}\right] \\ & =
\left[ \left( \restr{\alpha}{C_{n+k}(X', Y';\F)} \otimes \restr{\alpha}{C_{n+k}(X', Y';\F)} \right) \Delta_{n-k}(-) \right] \\ & =
Sq^k \circ \rho \big( [\alpha] \big)
\end{align*}
as claimed.
\end{comment}








% Please compare with the idealized Klein bottle studied in \cref{f:flat Klein bottle absolute}.
% The two longest bars in $\mathcal H^2_R$ correspond to the two most prominent $\mathcal H_1$ bars as found in the persistent homology barcode, while the longest bar in $\mathcal H^3_R$ corresponds to the most prominent $\mathcal H_2$ bar.
% Our implementation detects a single $Sq^1$ bar in this dataset, which is born with one of the two $\mathcal H^2_R$ bars and dies with the long $\mathcal H^3_R$ bar.
% This Steenrod bar would give rise to one in persistent absolute cohomology in a similar way as for our synthetic Klein bottle example in \cref{ss:flat Klein bottle}.
% However, in view of the discussions in \cref{ss:duality} and \cref{ss:truncations}, this does not amount to a fully rigorous characterization of the true persistent absolute cohomology barcode below the chosen distance threshold, once the latter is dropped from the computation.
% Fully settling this issue goes beyond the scope of this example.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{aux/figures/cyclo-octane_subsampled_barcodes.pdf}
%     \caption{Persistent relative cohomology barcode and $Sq^1$ Steenrod barcode for a subsample of size $800$ of the ``Klein bottle component'' of the conformational space of cyclo-octane, using a Vietoris--Rips filtration with dimension and distance thresholds at $3$ and $1.5$ respectively.
%     To reduce clutter, in the persistent relative cohomology barcode we do not show any bars in dimensions $0$ and $1$, and also do not show infinite bars in dimension $3$ (whose births would lie between $R \approx 1.03$ and the threshold $R = 1.5$).}
%     \label{fig:cyclo-octane subsampled}
% \end{figure}
